Long-Baseline Neutrino Facility (LBNF) and Deep Underground Neutrino Experiment (DUNE) Conceptual Design Report Volume 1: The LBNF and DUNE Projects

This document presents the Conceptual Design Report (CDR) put forward by an international neutrino community to pursue the Deep Underground Neutrino Experiment at the Long-Baseline Neutrino Facility (LBNF/DUNE), a groundbreaking science experiment for long-baseline neutrino oscillation studies and for neutrino astrophysics and nucleon decay searches. The DUNE far detector will be a very large modular liquid argon time-projection chamber (LArTPC) located deep underground, coupled to the LBNF multi-megawatt wide-band neutrino beam. DUNE will also have a high-resolution and high-precision near detector.

==> common/acronyms-shared-vol2-4.tex <==
%%%%%%%%%%%%% PHYSICS AND DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%
\nomenclature{CC}{charged current (interaction)}
\nomenclature{DIS}{deep inelastic scattering}
\nomenclature{FSI}{final-state interactions}
\nomenclature{GEANT4}{GEometry ANd Tracking, a platform for the simulation of the passage of particles through matter using Monte Carlo methods} 
\nomenclature{GENIE}{Generates Events for Neutrino Interaction Experiments (an object-oriented neutrino Monte Carlo generator)} 
\nomenclature{MC}{Monte Carlo (detector simulation methods)}
\nomenclature{QE}{quasi-elastic (interaction)}

==> common/acronyms-vol2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% PHYSICS VOLUME list for acronyms below %%%%%%%%%%%%%%%
\nomenclature{BR}{branching ratio}
\nomenclature{DM}{dark matter}
\nomenclature{DSNB}{Diffuse Supernova Neutrino Background}
\nomenclature{GLoBES}{General Long-Baseline Experiment Simulator (software package)}
\nomenclature{L/E}{length-to-energy ratio}
\nomenclature{LRI}{long-range interactions}
\nomenclature{$M_{\odot}$}{solar mass}
\nomenclature{NC}{neutral current (interaction)}
\nomenclature{NH}{normal (mass) hierarchy}
\nomenclature{NSI}{nonstandard interactions}
\nomenclature{MSW}{Mikheyev-Smirnov-Wolfenstein (effect)}
\nomenclature{SME}{Standard-Model Extension}
\nomenclature{SUSY}{supersymmetry}
\nomenclature{WIMP}{weakly-interacting massive particle}


==> common/acronyms-vol4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%%%%

\nomenclature{CE}{Cold Electronics}
\nomenclature{COB}{cluster on-board (motherboards)} %?
\nomenclature{CRP}{Charge-Readout Planes }
\nomenclature{DRAM}{dynamic random access memory}
\nomenclature{FE}{front end (electronics)}
%\nomenclature{Fermilab (also FNAL)}{Fermi National Accelerator Laboratory (in Batavia, IL, the Near Site)}
%\nomenclature{FNAL}{see Fermilab}
\nomenclature{FPGA}{field programmable gate array} %?
\nomenclature{FGT}{Fine-Grained Tracker}
\nomenclature{FS}{full stream (data volumes)} %?
\nomenclature{LEM}{Large Electron Multiplier}
\nomenclature{LNG}{liquefied natural gas}
%\nomenclature{LNGS}{Laboratori Nazionali (National Laboratory) del Gran Sasso (in L'Aquila, Italy)}
%\nomenclature{MaVaNs}{mass varying neutrinos}
\nomenclature{MIP}{minimum ionizing particle}
\nomenclature{MTS}{Materials Test Stand}
\nomenclature{MuID}{muon identifier (detector)}
%\nomenclature{OPERA}{Oscillation Project with Emulsion-Racking Apparatus (experiment at LNGS)}
\nomenclature{NND}{(used only in Volume 4 Chapter 7) near neutrino detector, same as ND}
%\nomenclature{OD}{outer diameter}
\nomenclature{PD}{photon detection (system)}
\nomenclature{PMT}{photomultiplier tube}
\nomenclature{PPM/PPB/PPT}{parts per million/billion/trillion}
\nomenclature{RCE}{reconfigurable computing element}
\nomenclature{RIO}{reconfigurable input output}
\nomenclature{RPC}{resistive plate chamber}
\nomenclature{SiPM}{silicon photomultiplier}
\nomenclature{S/N}{signal-to-noise (ratio)}
\nomenclature{SSP}{SiPM signal processor}
\nomenclature{SBN}{Short-Baseline Neutrino program (at Fermilab)}
\nomenclature{STT}{straw tube tracker}
%\nomenclature{SURF (also Sanford Lab)}{Sanford Underground Research Facility (in Lead, SD, the Far Site)}
\nomenclature{TR}{transition radiation}
%\nomenclature{W}{Watt (also mW, kW, MW) }
%\nomenclature{WA105}{Single-Phase LArTPC and the Long Baseline Neutrino Observatory Demonstration}
\nomenclature{WLS}{wavelength shifting}
\nomenclature{ZS}{zero suppression}


==> common/acronyms.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% COMMON list for acronyms below %%%%%%%%%%%%%%%
\nomenclature{$\mathcal{O}(n)$}{of order $n$}
\nomenclature{3D}{3 dimensional (also 1D, 2D, etc.)} % not phys
\nomenclature{CDR}{Conceptual Design Report}
\nomenclature{CF}{Conventional Facilities}
\nomenclature{CP}{product of charge and parity transformations}
\nomenclature{CPT}{product of charge, parity and time-reversal transformations}
\nomenclature{CPV}{violation of charge and parity symmetry}
\nomenclature{DAQ}{data acquisition}
\nomenclature{DOE}{U.S. Department of Energy}
\nomenclature{DUNE}{Deep Underground Neutrino Experiment}
\nomenclature{ESH}{Environment, Safety and Health}
\nomenclature{eV}{electron-Volt, unit of energy (also keV, MeV, GeV, etc.)}
\nomenclature{FD}{far detector}
\nomenclature{FGT}{Fine-Grained Tracker}
\nomenclature{FSCF}{far site conventional facilities}
\nomenclature{NSCF}{near site conventional facilities}
\nomenclature{GUT}{grand unified theory}
\nomenclature{\ktyr}{exposure (without beam), expressed in kilotonnes times years}
\nomenclature{\ktMWyr}{exposure, expressed in kilotonnes $\times$ megawatts $\times$ years} 
\nomenclature{L}{level, indicates depth in feet underground at the far site, e.g., 4850L}
\nomenclature{LAr}{liquid argon}
\nomenclature{LArTPC}{liquid argon time-projection chamber}
\nomenclature{LBL}{long-baseline (physics)}
\nomenclature{LBNF}{Long-Baseline Neutrino Facility}
\nomenclature{MH}{mass hierarchy}
\nomenclature{MI}{Main Injector (at Fermilab)}
\nomenclature{ND}{near neutrino detector}
\nomenclature{NDS}{Near Detector Systems; refers to the collection of detector systems at the near site }
\nomenclature{near detector}{except in Volume 4 Chapter 7, this refers to the \textit{neutrino} detector system in the NDS}
\nomenclature{NND}{(used only in Volume 4 Chapter 7) near neutrino detector, same as ND}
\nomenclature{POT}{protons on target}
\nomenclature{QA}{quality assurance}
\nomenclature{SM}{Standard Model of particle physics}
\nomenclature{t}{metric ton, written \textit{tonne} (also kt)}
\nomenclature{TPC}{time-projection chamber (not used as `total project cost' in the CDR)}

%%%%%%%%%%%%%%%%%%%%%%%%% PROJECT VOLUME list for acronyms below %%%%%%%%%%%%%%%
\nomenclature{L1, L2, ...}{WBS level within the LBNF and DUNE Projects, where the overall Project is L1}
\nomenclature{MOU}{memorandum of understanding}
\nomenclature{SDSTA}{South Dakota Science and Technology Authority}
\nomenclature{WBS}{Work Breakdown Structure}


%%%%%%%%%%%%%%%%%%%%%%%%% PHYSICS VOLUME list for acronyms below %%%%%%%%%%%%%%%
\nomenclature{BR}{branching ratio}
\nomenclature{DM}{dark matter}
\nomenclature{DSNB}{Diffuse Supernova Neutrino Background}
\nomenclature{GLoBES}{General Long-Baseline Experiment Simulator (software package)}
\nomenclature{L/E}{length-to-energy ratio}
\nomenclature{LRI}{long-range interactions}
\nomenclature{$M_{\odot}$}{solar mass}
\nomenclature{NC}{neutral current (interaction)}
\nomenclature{NH}{normal (mass) hierarchy}
\nomenclature{NSI}{nonstandard interactions}
\nomenclature{MSW}{Mikheyev-Smirnov-Wolfenstein (effect)}
\nomenclature{SME}{Standard-Model Extension}
\nomenclature{SUSY}{supersymmetry}
\nomenclature{WIMP}{weakly-interacting massive particle}

%%%%%%%%%%%%% PROJECT AND PHYSICS VOLUME list for acronyms below %%%%%%%%%%%%
\nomenclature{C.L.}{confidence level}

%%%%%%%%%%%%% PROJECT AND DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%

\nomenclature{APA}{anode plane assembly} 
\nomenclature{BLM}{(in Volume 4) beamline measurement (system); (in Volume 3) beam loss monitor}
\nomenclature{CPA}{cathode plane assembly}
\nomenclature{ECAL}{electromagnetic calorimeter}
\nomenclature{GAr}{gaseous argon}
\nomenclature{HV}{high voltage}

%%%%%%%%%%%%% PHYSICS AND DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%
\nomenclature{CC}{charged current (interaction)}
\nomenclature{DIS}{deep inelastic scattering}
\nomenclature{FSI}{final-state interactions}
\nomenclature{GEANT4}{GEometry ANd Tracking, a platform for the simulation of the passage of particles through matter using Monte Carlo methods} 
\nomenclature{GENIE}{Generates Events for Neutrino Interaction Experiments (an object-oriented neutrino Monte Carlo generator)} 
\nomenclature{MC}{Monte Carlo (detector simulation methods)}
\nomenclature{QE}{quasi-elastic (interaction)}

%%%%%%%%%%%%%%%%%%%%%%%%% DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%%%%

\nomenclature{CE}{Cold Electronics}
\nomenclature{COB}{cluster on-board (motherboards)} %?
\nomenclature{CRP}{Charge-Readout Planes }
\nomenclature{DRAM}{dynamic random access memory}
\nomenclature{FE}{front end (electronics)}
%\nomenclature{Fermilab (also FNAL)}{Fermi National Accelerator Laboratory (in Batavia, IL, the Near Site)}
%\nomenclature{FNAL}{see Fermilab}
\nomenclature{FPGA}{field programmable gate array} %?
\nomenclature{FGT}{Fine-Grained Tracker}
\nomenclature{FS}{full stream (data volumes)} %?
\nomenclature{LEM}{Large Electron Multiplier}
%\nomenclature{LNGS}{Laboratori Nazionali (National Laboratory) del Gran Sasso (in L'Aquila, Italy)}
%\nomenclature{MaVaNs}{mass varying neutrinos}
\nomenclature{MIP}{minimum ionizing particle}
\nomenclature{MTS}{Materials Test Stand}
\nomenclature{MuID}{muon identifier (detector)}
%\nomenclature{OPERA}{Oscillation Project with Emulsion-Racking Apparatus (experiment at LNGS)}
\nomenclature{octant}{any of the eight parts into which 4$\pi$ is divided by three mutually perpendicular axes}
%\nomenclature{OD}{outer diameter}
\nomenclature{PD}{photon detection (system)}
\nomenclature{PMT}{photomultiplier tube}
\nomenclature{RCE}{reconfigurable computing element}
\nomenclature{RIO}{reconfigurable input output}
\nomenclature{RPC}{resistive plate chamber}
\nomenclature{SiPM}{silicon photomultiplier}
\nomenclature{S/N}{signal-to-noise (ratio)}
\nomenclature{SSP}{SiPM signal processor}
\nomenclature{STT}{straw tube tracker}
%\nomenclature{SURF (also Sanford Lab)}{Sanford Underground Research Facility (in Lead, SD, the Far Site)}
\nomenclature{TR}{transition radiation}
%\nomenclature{W}{Watt (also mW, kW, MW) }
%\nomenclature{WA105}{Single-Phase LArTPC and the Long Baseline Neutrino Observatory Demonstration}
\nomenclature{WLS}{wavelength shifting}
\nomenclature{ZS}{zero suppression}

\fixme{Do we need GVKM, SNO, QCD,  PANDORA,  aTCA and microTCA, AMC, MCH, CPU, GPU, VHDL, OpenCL, PTP, Sync-E, GPS, IEEE, WR}







==> common/init-annex.tex <==
% This should be \input first thing after \begin{document}


\pagestyle{titlepage}

\begin{center}
  {\Huge  \thedoctitle}

  \vspace{10mm}

 {\LARGE \thedocsubtitle}

  \vspace{15mm}

\titleextra

  \vspace{10mm}
  \today
\end{center}

\clearpage

\pagestyle{plain} 

\renewcommand{\familydefault}{\sfdefault}
\renewcommand{\thepage}{\roman{page}}
\setcounter{page}{0}
\cleardoublepage

\setcounter{tocdepth}{3}
\textsf{\tableofcontents}
\clearpage


\textsf{\listoffigures}
\clearpage

\textsf{\listoftables}
\clearpage

%For acronym list to appear just after TOC
%\printnomenclature
\cleardoublepage

\iffinal\else
\textsf{\listoftodos}
\clearpage
\fi

\renewcommand{\thepage}{\arabic{page}}
\setcounter{page}{1}

\pagestyle{fancy}

% Set how header/footers look
\renewcommand{\chaptermark}[1]{%
\markboth{Chapter \thechapter:\ #1}{}}
\fancyhead{}
\fancyhead[RO,LE]{\textsf{\footnotesize \thechapter--\thepage}}
\fancyhead[LO,RE]{\textsf{\footnotesize \leftmark}}

\fancyfoot{}
\fancyfoot[RO]{\textsf{\footnotesize LBNF/DUNE Conceptual Design Report}}
\fancyfoot[LO]{\textsf{\footnotesize \thedoctitle}}
\fancypagestyle{plain}{}

\renewcommand{\headrule}{\vspace{-4mm}\color[gray]{0.5}{\rule{\headwidth}{0.5pt}}}



==> common/intro.tex <==
% Intro shared by all subsections

\section{An International Physics Program}

The global neutrino physics community is developing a multi-decade
physics program to measure unknown parameters of the Standard Model of
particle physics and search for new phenomena.  The program will be carried out as an international,
leading-edge, dual-site experiment for neutrino science and proton decay studies, which 
is known as the Deep Underground Neutrino Experiment (DUNE).
The detectors for this experiment will be designed, built, commissioned and operated by the international DUNE Collaboration. The facility required to support this experiment, the Long-Baseline Neutrino Facility (LBNF), is hosted by Fermilab and its design and construction is organized as a DOE/Fermilab project incorporating international partners. Together LBNF and DUNE will comprise the world's highest-intensity neutrino beam at Fermilab, in Batavia, IL, a high-precision near detector on the Fermilab site, a massive liquid argon time-projection chamber (LArTPC) far detector installed deep underground at the Sanford Underground Research Facility (SURF) \SI{1300}{\km} away in Lead, SD, and all of the conventional and technical facilities necessary to support the beamline and detector systems. 


The strategy for executing the experimental program presented in this Conceptual 
Design Report (CDR) has been developed to meet the requirements 
set out in the P5 report~\cite{p5report} and takes into account the recommendations of the European Strategy for Particle Physics~\cite{ESPP-2012}. It adopts a model where U.S. and international funding agencies 
share costs on the DUNE detectors, and CERN and other participants provide in-kind contributions 
to the supporting infrastructure of LBNF. LBNF and DUNE will be tightly coordinated as DUNE collaborators 
design the detectors and infrastructure that will carry out the scientific program.
  
The scope of LBNF is
\begin{itemize}
\item an intense neutrino beam aimed at the far site,
\item conventional facilities at both the near and far sites, and
\item cryogenics infrastructure to support the DUNE detector at the far site.
\end{itemize}

The DUNE detectors include
\begin{itemize}
\item a high-performance neutrino detector and beamline  
measurement system
located a few hundred meters downstream of the neutrino source, and
\item a massive liquid argon time-projection chamber (LArTPC) neutrino detector located deep underground at the far site.
\end{itemize}

With the facilities provided by LBNF and the detectors provided by
DUNE, the DUNE Collaboration proposes to mount a focused attack on the
puzzle of neutrinos with broad sensitivity to neutrino oscillation
parameters in a single experiment.  The focus of the scientific
program is the determination of the neutrino mass hierarchy and the
explicit demonstration of leptonic CP violation, if it exists, by
precisely measuring differences between the oscillations of muon-type
neutrinos and antineutrinos into electron-type neutrinos and
antineutrinos, respectively. Siting the far detector deep underground
will provide exciting additional research opportunities in nucleon
decay, studies utilizing atmospheric neutrinos, and neutrino
astrophysics, including measurements of neutrinos from a core-collapse
supernova should such an event occur in our galaxy during the
experiment's lifetime.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The LBNF/DUNE Conceptual Design Report Volumes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{A Roadmap of the CDR}

The LBNF/DUNE CDR describes the proposed physics program and 
technical designs at the conceptual design stage.  At this stage, the design is
still undergoing development and the CDR therefore presents a \textit{reference design} 
for each element as well as \textit{alternative designs} that are under consideration.

The CDR is composed of four volumes and is supplemented by several annexes that 
provide details on the physics program and technical designs. The volumes are as follows

\begin{itemize}
\item \volintro{}\cite{cdr-vol-1} provides an executive summary of and strategy for the experimental 
program and introduces the CDR.
\item \volphys{}\cite{cdr-vol-2} outlines the scientific objectives and describes the physics studies that 
the DUNE Collaboration will undertake to address them.
\item \vollbnf{}\cite{cdr-vol-3} describes the LBNF Project, which includes design and construction of the 
beamline at Fermilab, the conventional facilities at both Fermilab and SURF, and the cryostat
 and cryogenics infrastructure required for the DUNE far detector.
\item \voldune{} describes the DUNE Project, which includes the design, construction and 
commissioning of the near and far detectors. 
\end{itemize}

More detailed information for each of these volumes is provided in a set of annexes listed on LBNF and DUNE's shared  \href{https://web.fnal.gov/project/LBNF/SitePages/Proposals%20and%20Design%20Reports.aspx}{\textit{Proposals and Design Reports} page}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{About this Volume}  <----- follows in overview chapter file of indiv volume



==> compileitduneprint <==
#!/bin/sh
pdflatex "\def\isfinal{1} \input{$1}"
pdflatex "\def\isfinal{1} \input{$1}"
bibtex $1
pdflatex "\def\isfinal{1} \input{$1}"
pdflatex "\def\isfinal{1} \input{$1}"
makeindex $1.nlo -s nomencl.ist -o $1.nls
pdflatex "\def\isfinal{1} \input{$1}"
pdflatex "\def\isfinal{1} \input{$1}"


==> tables/zs-volume-table.tex <==
% do not edit, this is generated by dune-params
% per 40kt DUNE
% name, event rate, event size, data rate, annual data volume
\begin{tabular}[h]{r|r|r|r|r}
\hline
source & event rate & event size & data rate & annual data volume \\
\hline
$^{39}Ar$ & \SI[round-mode=places,round-precision=1]{37.8}{\mega\hertz} & \SI[round-mode=places,round-precision=0]{36.0}{\byte} &
\SI[round-mode=places,round-precision=1]{1.3608}{\giga\byte\per\second} &  \SI[round-mode=places,round-precision=0]{42.9426648664}{\peta\byte}\\
\hline
cosmic-$\mu$ & \SI[round-mode=places,round-precision=3]{0.258947264}{\hertz} &
\SI[round-mode=places,round-precision=1]{50.0}{\kilo\byte} & \SI[round-mode=places,round-precision=1]{12.9473632}{\kilo\byte\per\second} &
\SI[round-mode=places,round-precision=0]{408.57898207}{\giga\byte} \\
\hline
beam-$\nu$ & \SI[round-mode=places,round-precision=0]{10524.2348126}{\per\year} & \SI[round-mode=places,round-precision=1]{10.0}{\mega\byte} &
\SI{3.335}{\kilo\byte\per\second} & \SI[round-mode=places,round-precision=0]{105.242348126}{\giga\byte} \\
\hline
SNB cand. (ZS) & \SI[round-mode=places,round-precision=0]{12.0}{\per\year} & \SI[round-mode=places,round-precision=1]{13.608}{\giga\byte} &
\SI[round-mode=places,round-precision=0]{5174.64851079}{\byte\per\second} & \SI[round-mode=places,round-precision=0]{163.296}{\giga\byte} \\
SNB cand. (FS) & \SI[round-mode=places,round-precision=0]{12.0}{\per\year} & \SI[round-mode=places,round-precision=1]{46.08}{\tera\byte} &
\SI[round-mode=places,round-precision=1]{17.5226192958}{\mega\byte\per\second} & \SI[round-mode=places,round-precision=0]{552.96}{\tera\byte} \\
\hline
\end{tabular}
